The VLBA Imaging and Polarimetry Survey at 5 GHz

We present the first results of the VLBA Imaging and Polarimetry Survey (VIPS), a 5 GHz VLBI survey of 1,127 sources with flat radio spectra. Through automated data reduction and imaging routines, we have produced publicly available I, Q, and U images and have detected polarized flux density from 37% of the sources. We have also developed an algorithm to use each source's I image to automatically classify it as a point-like source, a core-jet, a compact symmetric object (CSO) candidate, or a complex source. The mean ratio of the polarized to total 5 GHz flux density for VIPS sources with detected polarized flux density ranges from 1% to 20% with a median value of about 5%. We have also found significant evidence that the directions of the jets in core-jet systems tend to be perpendicular to the electric vector position angles (EVPAs). The data is consistent with a scenario in which ~24% of the polarized core-jets have EVPAs that are anti-aligned with the directions of their jet components and which have a substantial amount of Faraday rotation. In addition to these initial results, plans for future follow-up observations are discussed.

==> tab3.tex <==
\begin{deluxetable}{lcc}
\tablecolumns{3}
\tablewidth{0pc}
\tablecaption{Summary of Source Types}
\tablehead{
\colhead{Type} & \colhead{N} & \colhead{N$_{pol}$/N} \\
\colhead{(1)} & \colhead{(2)} & \colhead{(3)}}

\startdata
PS & 276 & 31$\pm$4\% \\
SJET & 241 & 36$\pm$5\% \\
LJET & 471 & 41$\pm$4\% \\
CSO & 103 & 15$\pm$4\% \\
CPLX & 17 & 11$\pm$8\% \\
ND & 11 & \nodata \\
\enddata

\tablecomments{Col.\ (1): Source type determined using the ``by-eye'' reclassifications of the automatic classifications where applicable (see \S 2.3).  Col.\ (2): Number of sources within the class listed in Col.\ (1).  Col.\ (3): Percentage of sources with detected ($>5\sigma$) polarized flux within the class listed in Col.\ (1) (not including sources with only CJF or VIPS pilot data).} 
\label{classes}
\end{deluxetable}

